Stability of Neural Networks on Riemannian Manifolds

Convolutional Neural Networks (CNNs) have been applied to data with underlying non-Euclidean structures and have achieved impressive successes. This brings the stability analysis of CNNs on non-Euclidean domains into notice because CNNs have been proved stable on Euclidean domains. This paper focuses on the stability of CNNs on Riemannian manifolds. By taking the Laplace-Beltrami operators into consideration, we construct an $\alpha$-frequency difference threshold filter to help separate the spectrum of the operator with an infinite dimensionality. We further construct a manifold neural network architecture with these filters. We prove that both the manifold filters and neural networks are stable under absolute perturbations to the operators. The results also implicate a trade-off between the stability and discriminability of manifold neural networks. Finally we verify our conclusions with numerical experiments in a wireless adhoc network scenario.

==> proof.tex <==
\section{Proof of Theorem \ref{thm:stability_filter}}
\begin{proof}
Begin with the definition of spectral convolution operators in \eqref{eqn:operator}, we can rewrite the norm difference between two outputs as:
\begin{align}
   \nonumber & \left\| H(\ccalL) f  - H(\ccalL+A)f\right\|
    \\
  \nonumber  & = \| \sum_{i\in\ccalD} h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i +\sum_{n\in\ccalN} h_n \langle f, E_n  \rangle E_n \\
    & - \sum_{i\in\ccalD} h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i  -\sum_{n\in\ccalN} h_n \langle f, E'_n  \rangle E'_n \| 
  \\ \nonumber & \leq  \left\| \sum_{i\in \ccalD} h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i  - \sum_{i\in \ccalD} h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i \right\| \\
  & + \sum_{n\in\ccalN}\|h_n\| \left\|  \langle f, E_n  \rangle E_n -   \langle f, E'_n  \rangle E'_n  \right\|  \label{eqn:HS}
  % &\leq \left\| \sum_{n\in \ccalD_1} h(\lambda_{n}) \langle f, \bm\phi_n \rangle \bm\phi_n -  h(\lambda'_{n}) \langle f, \bm\phi'_n \rangle \bm\phi'_n \right\| + \left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -  \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} \right\| 
    %\\
    %&\leq \left\| \sum_{n\in \ccalD_1} h(\lambda_{n}) \langle f, \bm\phi_n \rangle \bm\phi_n -  h(\lambda'_{n}) \langle f, \bm\phi'_n \rangle \bm\phi'_n \right\| + \{\|h(E_{\bar\ccalD_1})\|,\|h(E'_{\overline{\ccalD}})\|\} \|\langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} - \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} \| 
\end{align}
%The decomposition in \eqref{eqn:decompose} results from the boundedness of filter function. 
$E_{n}$ is column space of eigenfunctions $[\bm\phi_i]_{i\in\ccalN_n}$ while $E'_{n}$ is column space of eigenfunctions $[\bm\phi'_i]_{i\in\ccalN_n}$.

For the first term in \eqref{eqn:HS}, with the triangle inequality the norm difference can then be written as:
\begin{align}
 & \nonumber \left\| \sum_{i\in \ccalD} h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i  -  h(\lambda'_i )  \langle f, \bm\phi'_i \rangle \bm\phi'_i \right\| \\
 & =\|\sum_{i \in \ccalD}  h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i -  h(\lambda_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i +  h(\lambda_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i\nonumber \\
  & \qquad \qquad \qquad \qquad \qquad \qquad\qquad \quad- h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i \| \\
 &\nonumber \leq \left\|\sum_{i \in \ccalD_1}  h(\lambda_i  \langle f, \bm\phi_i \rangle \bm\phi_i -  h(\lambda_i ) \langle f, \bm\phi'_i \rangle \bm\phi'_i\right\|\\
 & \qquad \qquad \quad+ \left\|\sum_{i \in \ccalD_1} h(\lambda_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i -  h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i \right\|\\
 &\leq \left\| \sum_{i \in \ccalD_1}  h(\lambda_i)\left( \langle f, \bm\phi_i \rangle\bm\phi_i-\langle f, \bm\phi_i \rangle\bm\phi'_i +\langle f, \bm\phi_i \rangle\bm\phi'_i - \langle f, \bm\phi'_i \rangle \bm\phi'_i \right) \right\| \nonumber \\
 & \qquad \qquad \qquad\qquad+ \left\|\sum_{i \in \ccalD_1}  (h(\lambda_i ) -h(\lambda'_i)  \langle f, \bm\phi'_i \rangle \bm\phi'_i  \right\| \\
 & \leq \left\| \sum_{i \in \ccalD_1} h(\lambda_i )\langle f, \bm\phi_i \rangle (\bm\phi_i - \bm\phi'_i ) \right\| +\left\|  \sum_{i \in \ccalD_1}  h(\lambda_i )\langle f, \bm\phi_i - \bm\phi'_i  \rangle \bm\phi'_i \right\|\nonumber \\ 
 &\qquad \qquad \qquad\qquad + \left\|\sum_{i \in \ccalD_1}  (h(\lambda_i ) -h(\lambda'_i) ) \langle f, \bm\phi'_i \rangle \bm\phi'_i  \right\|\label{eqn:3}
    % \\
    % &\leq 2\sum_{n }  \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| + \sum_{n }  \left\|h(\lambda_{n}) -h(\lambda'_n) \right\|  \left\| f \right\| 
    % &\left\| \sum_{n\in C} h(\lambda_n)\langle f, \bm\phi_n \rangle (\bm\phi_n-\bm\phi'_n) \right\| +\left\|  \sum_{n\in C}   h(\lambda_n)\langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\|+ \left\|\sum_{n\in C}   (h(\lambda_{n}) -h(\lambda'_n) ) \langle f, \bm\phi'_n \rangle \bm\phi'_n  \right\|
    \\
 &\leq 2 \sum_{i \in \ccalD_1}    \left\|h(\lambda_i )\right\| \left\|f\right\| \left\|\bm\phi_i-\bm\phi'_i \right\| + \sum_{i \in \ccalD_1}   \left\| (h(\lambda_i ) -h(\lambda'_i ) )\right\|\|f\| \label{eqn:2}
\end{align}

For the second term in \eqref{eqn:HS}, similarly with the triangle inequality, we have:
\begin{align}
\sum_{n\in\ccalN}\|h_n\| \left\|  \langle f, E_n  \rangle E_n -   \langle f, E'_n  \rangle E'_n  \right\| \leq 2\sum_{n\in\ccalN} \|E_n-E'_n\|
\end{align}
%\begin{align}
%&\left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -  \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} \right\| \\ 
%&\leq \left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -   \underline{h}(E'_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} +  \underline{h}(E'_{\bar\ccalD_1}) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} - \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1}   \right\| \\ 
%& \leq \left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -   \underline{h}(E'_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1}\right\| + \left\|   \underline{h}(E'_{\bar\ccalD_1}) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} - \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1}   \right\| \\
%& \leq \left\|  \overline{h}(E_{\bar\ccalD_1}) -  \underline{h}(E'_{\bar\ccalD_1}) \right\| \|f\| + 2\left\| E_{\bar\ccalD_1} - E'_{\bar\ccalD_1}  \right\|\|f\| \\
%&\leq 2\left\| E_{\bar\ccalD_1} - E'_{\bar\ccalD_1}  \right\|\|f\|
%\end{align}

% The first and second terms can be analyzed separately in two parts. We design the operator in the form that $h(\lambda_n)$ is constant for $\lambda_n>c$. Therefore it can be rewritten as:
% \begin{align}
% &\left\| \sum_{n } h(\lambda_n)\langle f, \bm\phi_n \rangle (\bm\phi_n-\bm\phi'_n) \right\| +\left\|  \sum_{n }  h(\lambda_n)\langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\| \\
% &\leq \left\| \sum_{n=1 }^\bbarM h(\lambda_n)\| f\| \|\bm\phi_n\|   (\bm\phi_n-\bm\phi'_n) \right\| + \left\| \sum_{n=\bbarM+1}^\infty h(\lambda_n)\|f\| \|\bm\phi_n\| (\bm\phi_n-\bm\phi'_n) \right\| + \nonumber\\
% &\qquad \qquad \qquad \qquad\qquad \qquad\left\|  \sum_{n=1 }^\bbarM h(\lambda_n)\|f\| \|\bm\phi_n-\bm\phi'_n \| \bm\phi'_n \right\|+\left\|  \sum_{n=\bbarM+1 }^\infty  h(\lambda_n)\langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\|  \\
% &\leq 2 \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| +\left\| h(\lambda) \|f\|\sum_{n=\bbarM+1}^\infty(\bm\phi_n-\bm\phi'_n) \right\| + \left\| h(\lambda)\sum_{n=\bbarM+1}^\infty \langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\|\\
% & \leq 2 \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| + \|h(\lambda)\|\|f\| \left\|\sum_{n=\bbarM+1}^\infty (\bm\phi_n-\bm\phi'_n)\right\| + \|h(\lambda)\| \sum_{n=\bbarM+1}^\infty \langle f, \bm\phi_n-\bm\phi'_n \rangle 
% \label{eqn:1}\\
% & \leq 2 \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| +  2\|h(\lambda)\|\|f\|
% \left\|\sum_{n=\bbarM+1}^\infty (\bm\phi_n-\bm\phi'_n)\right\|.
% \label{eqn:2}
% \end{align}
% From \eqref{eqn:1} to \eqref{eqn:2}, this is due to the linearity of inner products. 

% By grouping eigenvalues that are close enough, i.e. $ \ccalC = \{ i\leq \bbarM: \min\{ |\lambda_i-\lambda'_{i+1}|, |\lambda_i-\lambda'_{i-1}|, |\lambda'_i-\lambda_{i+1}|, |\lambda'_i-\lambda_{i-1}| \} > \delta \} $, we can decompose the first item as:
% \begin{align}
%     \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\|= \sum_{n\in \ccalC} \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| + \max\limits_{i\in \bar\ccalC} \left\|h(\lambda_i)\right\|\left\|f\right\| \left\| E_{\bar\ccalC}  -E'_{\bar\ccalC}\right\|
% \end{align}
Now we need to include two important lemmas to analyze the influence on eigenvalues and eigenspaces caused by the perturbation.
\begin{lemma}\label{lem:eigenvalue_absolute}[Weyl's Theorem]
The eigenvalues of operators $\ccalL$ and $\ccalL'$ satisfy:
\begin{equation}
|\lambda_n-\lambda'_n|\leq \|\bbA\|\leq \epsilon.
\end{equation}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:eigenvalue_absolute}]
First assume that $\ccalL$ and $\bbA$ are symmetric operators. Let $\lambda_1\leq \lambda_2\leq \dots\leq \lambda_n\leq \cdots$ be the eigenvalues arranged in the ascending order. For each subspace $T$ of the manifold, define:
\begin{align}
    \lambda[\ccalL, T] =\min_{u\in T, \|u\|=1} \langle \ccalL, u \rangle.
\end{align}
The minimax principle asserts that:
\begin{align}
    \lambda_n(\ccalL)=\max_{codim T = n-1}\lambda[\ccalL, T]=\max_{codim \leq n-1} \lambda[\ccalL, T].
\end{align}
Each $u$ has the expansion:
\begin{align}
    u=\sum \xi_n\bm\phi_n, \quad \|u\|^2=\sum |\xi_n|^2.
\end{align}
Then:
\begin{align}
    \ccalL u=\sum \xi_n \ccalL \bm\phi_n,\quad \langle \ccalL u,u \rangle =\sum \lambda_n(\ccalL) |\xi_n|^2.
\end{align}
Therefore,
\begin{align}
    \lambda_1(\ccalL) \leq  \frac{\langle \ccalL u, u\rangle }{\|u\|^2} \leq \max_n\lambda_n(\ccalL).
\end{align}
Then for any $1\leq k $, we have:
\begin{align}
    \lambda_k(\ccalL+ \bbA) &=\max_{codim T\leq n-1} \min_{ u\in T, \|u\|=1}  \langle (\ccalL + \bbA) u, u\rangle \\
    & = \max_{codim T\leq n-1} \min_{ u\in T, \|u\|=1} \left \langle  \ccalL  u, u\rangle + \langle \bbA u, u\rangle   \right)\\
    & \geq \max_{codim T\leq n-1} \min_{  u\in T, \|u\|=1}  \left\langle  \ccalL  u, u\rangle   + \lambda_1(\bbA) \right)\\
    & = \lambda_1(\bbA)+ \max_{codim T\leq n-1} \min_{  u\in T, \|u\|=1 } \langle  \ccalL  u, u\rangle  \\
    & = \lambda_k(\ccalL)+\lambda_1(\bbA).
\end{align}
Similarly, we can have $\lambda_k(\ccalL+ \bbA) \leq \lambda_k(\ccalL)+ \max_n\lambda_n(\bbA)$. This leads to $\lambda_1(\bbA)\leq \lambda_k(\ccalL + \bbA )-\lambda_k(\ccalL) \leq \max_n\lambda_n(\bbA)$.
\end{proof}

To measure the difference of eigenspaces, 
\begin{lemma}[Davis-Kahan $\sin\theta$ Theorem]\label{lem:davis-kahan}
Suppose the spectra of $\ccalL$ and $\ccalL'$ are partitioned as $\sigma\bigcup\Sigma$ and $\omega\bigcup \Omega$ respectively, with $\sigma\bigcap \Sigma=\emptyset$ and $\omega\bigcap\Omega=\emptyset$. Then we have:
\begin{equation}
\|E_\ccalL(\sigma)-E_{\ccalL'}(\omega)\|\leq \frac{\pi}{2}\frac{\|(\ccalL'-\ccalL)E_\ccalL(\sigma)\|}{d}\leq \frac{\pi}{2}\frac{\|(\ccalL'-\ccalL)\|}{d},
\end{equation}
where $d$ satisfies: $\min_{x\in\sigma,y\in\Omega}|x-y|\geq d$ and $\min_{x\in\Sigma,y\in\omega}|x-y|\geq d$.
\end{lemma}


For the first term in \eqref{eqn:2}, we employ Lemma \ref{lem:davis-kahan} and therefore we have $\sigma=\lambda_n$ and $\omega=\lambda'_n$, for $n\in C$ we can have: 
\begin{align}
\left\| \bm\phi_n -\bm\phi'_n\right\| \leq \frac{\pi}{2} \frac{\|\bbA\|}{\delta}.
\end{align}

Similarly, for the second term in \eqref{eqn:HS} we have $\sigma=\{\lambda_i\}_{i\in\ccalN_n}$ and $\omega=\{\lambda'_i\}_{i\in\ccalN_n}$, 
\begin{align}
\left\| E_{n}  -E'_{n}\right\| \leq \frac{\pi}{2} \frac{\|\bbA\|}{\delta}.
\end{align}

The second term in \eqref{eqn:2} can be bounded by the Lipschitz continuity of $h$ combined with Lemma \ref{lem:eigenvalue_absolute}:
\begin{align}
\|\sum_{i\in\ccalD }   (h(\lambda_{i}) -& h(\lambda'_i) ) \langle f, \bm\phi'_i \rangle \bm\phi'_i  \| \nonumber\\
&\leq \sum_{i\in\ccalD}\left\| (h(\lambda_{i}) -h(\lambda'_i) )\right\|\|f\| \\
&\leq \sum_{i\in\ccalD} C |\lambda_i - \lambda'_i |\|f\|\leq |\ccalD| C \epsilon\|f\|.
\end{align}

%For $h(\lambda_n)$ is a constant for $n>\bbarM$, we can construct this by summing the bandwidth-limited filter for $n\leq \bbarM$ and a low-pass filter $g(\lambda)$ with $g(\lambda_n)$  a constant for $n>\bbarM$ and 0 otherwise. The low-pass filter is stable because it can be seen as the sum of a constant filter and a high-pass filter with an opposite value. 
\end{proof}

\section{Proof of Theorem \ref{thm:stability_nn}}
The difference can therefore be written as:
 \begin{align}
 &\nonumber\| f_l^k - f_l^{'k} \|=\\
 &\left\|  \sigma\left( \sum_{g=1}^{K_{l-1}} H_l^{kg}(\ccalL) f_{l-1}^g\right) -  \sigma\left( \sum_{g=1}^{K_{l-1}} H_l^{'kg}(\ccalL') f_{l-1}^{'g}\right) \right\|.   
 \end{align}
 With the assumption that $\sigma$ is normalized Lipschitz, we have:
 \begin{align}
  \| f_l^k - f_l^{'k} \| &\leq \left\| \sum_{g=1}^{K_{l-1}}  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g}  \right\|\\
  &\leq \sum_{g=1}^{K_{l-1}} \left\|  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g} \right\|.
 \end{align}
 By adding and subtracting $H_l^{'kg}(\ccalL') f_{l-1}^{g}$ from each term, combined with the triangle inequality we can get:
 \begin{align}
 &\left\|  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g} \right\| \\
 &\leq \left\|  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{g} \right\| \\
 &+ \left\| H_l^{'kg}(\ccalL') f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g} \right\|.
 \end{align}
 The first term can be bounded with \eqref{eqn:stability_filter}. The second term can be decomposed by Cauchy-Schwartz inequality and bound for filter function as:
 \begin{align}
 \| f_{l}^k - f_l^{'k} \| \leq \sum_{g=1}^{K_{l-1}} C_{per} \epsilon \bbarM \| f_{l-1}^g\| + \sum_{g=1}^{K_{l-1}} \| f_{l-1}^g - f_{l-1}^{'g} \|.
 \end{align}
 To solve this recursion, we need to compute the bound for $\|f_l^k\|$. By the Lipschitz continuity of $\sigma$ and the fact that $\sigma(0)=0$, we can get:
 \begin{align}
 \| f_l^k \|&\leq \left\| \sum_{g=1}^{K_{l-1}} H_l^{kg}(\ccalL) f_{l-1}^{g}  \right\|\leq  \sum_{g=1}^{K_{l-1}}  \left\| H_l^{kg}(\ccalL)\right\|  \|f_{l-1}^{g}  \| 
 \\ &\leq   \sum_{g=1}^{K_{l-1}}   \|f_{l-1}^{g}  \| \leq \prod\limits_{l'=1}^{l-1} K_{l'} \sum_{g=1}^{K_0}\| f^g \|.
 \end{align}
 Insert this conclusion back to solve the recursion, we can get:
 \begin{align}
 \| f_{l}^k - f_l^{'k} \|\leq l C_{per}\epsilon \left( \prod\limits_{l'=1}^{l-1} K_{l'} \right) \sum_{g=1}^{K_0} \|f^g\|.
 \end{align}
 Replace $l$ with $L$ we can obtain:
 \begin{align}
 \|y-y'\|^2 \leq \sum_{f=1}^{K_L} \left( L C_{per}\epsilon \left( \prod\limits_{l'=1}^{L-1} K_{l'} \right) \sum_{g=1}^{K_0} \|f^g\| \right)^2.
 \end{align}
 With $F_0=F_L=1$ and $F_l=F$ for $1\leq l\leq L-1$, then:
  \begin{align}
 \|y-y'\|^2 \leq LF^{L-1} C_{per}\epsilon  \|f\| .
 \end{align}
 \section{Proof of Proposition \ref{prop:finite_num}}
 Here we study the eigendecomposition in the Dirichlet condition. We have the following result for the spectrum of operator $\ccalL$ from results in \cite{berard2006spectral}.
\begin{theorem}\label{thm:eigenvalue}
Let $\ccalM$ be a compact manifold, consider the Dirichlet eigenvalue problems. Then:
\begin{enumerate}
    \item The set of eigenvalue consists of an infinite sequence $0<\lambda_1\leq \lambda_2\leq \lambda_3\leq \cdots \rightarrow \infty$;
    \item Each eigenvalue has finite multiplicity and the eigenspaces corresponding to distinct eigenvalues are $L^2(\ccalM)$-orthogonal;
\end{enumerate}
\end{theorem}

The spectrum cannot be calculated explicitly in general. However, it is still possible to get an estimation of the spectrum. The following Weyl's law gives a characterization of how the spectrum behaves asymptotically.
\begin{theorem}[Weyl's Law]\label{thm:Weyl_law}
If $(\ccalM,g)$ is a compact Riemannian manifold of dimension $d$, then
\begin{equation}\label{eqn:Weyllaw}
    \lambda_k(\ccalM,g)\sim \frac{4\pi^2}{C_d^{2/d}} \left( \frac{k}{\text{Vol}(\ccalM,g)} \right)^{2/d}
\end{equation}
as $k\rightarrow \infty$, and $C_d$ denotes the volume of the unit ball of $\reals^n$.
\end{theorem}

==> stability of NN on Rie-manifolds-eusipco/conclusions.tex <==
%!TEX root = conference-stability.tex


In this paper, we have defined manifold convolutions and manifold neural networks. Considering the infinite dimensionality of Laplace-Beltrami operators. We import the definition of $\alpha$ frequency difference threshold filters to help separate the spectrum. By assigning a constant frequency response to the eigenvalues that are close enough, $\alpha$-FDT filters can be proved to be stable to absolute perturbations to the Laplacian operators. We further prove that the manifold neural networks built with $\alpha$-FDT filters are also stable under absolute perturbations. We conclude that there is a trade-off between the stability and discriminability. We further verified our results numerically with a power allocation problem in wireless adhoc networks.



==> stability of NN on Rie-manifolds-eusipco/filters_manifold.tex <==
%!TEX root = conference-stability.tex

{In order to characterize the stability properties of MNNs, we first have to study the stability of their main component --- the convolutional filter in \eqref{eqn:operator}. In particular, we analyze the stability of convolutional filters to absolute perturbations of the Laplace-Beltrami operator, which are specified in Definition \ref{defn:absolute_perturbations}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DEFINITION %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}[Absolute perturbations] \label{defn:absolute_perturbations}
Let $\ccalL$ be the Laplace-Beltrami operator of a Riemannian manifold $\ccalM$. An absolute perturbation of $\ccalL$ is defined as%We say that a Laplace-Beltrami operator $\ccalL'$ is its perturbed operator if it has the form: 
\begin{equation}\label{eqn:perturb}
\ccalL'=\ccalL+\bbA,
\end{equation}
where the absolute perturbation operator $\bbA$ is symmetric.
\end{definition}

%As per Definition \ref{defn:absolute_perturbations}, the Laplacian operator $\ccalL$ is perturbed to $\ccalL'$ according to \eqref{eqn:perturb}. 
The absolute perturbation model introduced in Definition \ref{defn:absolute_perturbations} only requires $\bbA$ to be symmetric. Thus, it is a rather generic perturbation model encompassing many different types of perturbations and, in particular, allowing to model a wide array of perturbations to the underlying manifold $\ccalM$.
%Give a perturbed manifold, we can always consider its Laplacian operator before and after the perturbation. 
%With some specific perturbation operators, the absolute perturbation model can be used to represent a wide array of perturbations to the underlying manifold.
%With regards to specific graph perturbations, note that they can be modeled as absolute graphon perturbations if, given a graph, we consider its induced graphon, and, given a graph perturbation, we consider its induced graphon representation [cf. equation (7)]. Since the absolute graphon perturbation model is very general, it can be used to represent a wide array of graph perturbations
%\red{L: Describe an absolute perturbation in words. You can also make a comment on how this perturbation model is general and allows modeling operator perturbations corresponding to a wide array of perturbations to the underlying manifold.}

\subsection{Frequency difference threshold (FDT) filters}

{Given the spectral decomposition of the Laplace-Beltrami operator \eqref{eqn:Laplacian}, we can expect an absolute perturbation of $\ccalL$ to spawn some sort of perturbation to the eigenvalues $\lambda_i$. Since the spectral convolution operation \eqref{eqn:operator} depends on the evaluation of $h(\lambda)$ at each $\lambda_i$, its stability analysis will depend on the individual effects of the perturbation on each of these eigenvalues. A challenge in the case of manifolds is that the spectrum of $\ccalL$ is infinite-dimensional, i.e., there is an infinite (albeit countable) number of eigenvalues $\lambda_i$. However, it is possible to show that these eigenvalues accumulate in certain parts of the spectrum. This is demonstrated in Proposition \ref{prop:finite_num}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% PROPOSITION %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proposition} \label{prop:finite_num}
Let $(\ccalM,g)$ be a $d$-dimensional Riemannian manifold with Laplacian-Beltrami operator $\ccalL$, and let $\lambda_k$ denote the eigenvalues of $\ccalL$. Let $C_1$ denote an arbitrary constant and let $C_d$ be the volume of the $d$-dimensional unit ball. For any $\alpha > 0$, there exists $N_1$ given by
\begin{equation}
    N_1=\lceil (\alpha d/C_1)^{d/(2-d)}(C_d \text{Vol}(\ccalM,g))^{2/(2-d)} \rceil
\end{equation}
such that, for all $k>N_1$, it holds that $$\lambda_{k+1}-\lambda_k\leq \alpha.$$
%\red{L: This proposition is a bit vague. Can you make it more specific? E.g., what is the spectrum behavior of the Laplacian operator on Riemannian manifolds?}
\end{proposition}
\begin{proof}
This is a direct consequence of Weyl's law \cite{arendt2009weyl}.
\end{proof}
%\red{L: If the proof of Prop. 1 is not too long, I would include it here. Especially if we make this a purely theoretical paper and don't add any experiments.}
%In the definition of convolutional filter in ..., we see that the manifold convolution operates in the frequency domain by scaling each of the signal's $i$-th spectral components by $h(\lambda_i)$. Thus, we can expect 
%

{Proposition \ref{prop:finite_num} is important because it suggests a strategy to mitigate the challenge posed by the infinite-dimensional spectrum of $\ccalL$. Since eigenvalues accumulate in certain parts of this spectrum, for $\alpha >0$ we can gather eigenvalues that are less than $\alpha$ apart in a \textit{finite} number of groups. This $\alpha$-separated spectrum, formalized in Definition \ref{def:alpha-spectrum}, is achieved by the so-called frequency difference threshold (FDT) filters introduced in Definition \ref{def:alpha-filter}.}

%is spectral separation can be achieved by applying 

%according to Def. X is can be ob 
%To obtain this spectral sep, we need a filter that

%This yields an $\alpha$-separated spectrum, a notion that we formalize Definition \ref{def:alpha-spectrum}. Importantly, o achieve this spectrum separation, } 

%We first define an $\alpha-$separated spectrum as:

%\red{L: These definitions are too long and maybe a little convoluted. Try to make them more concise. Check, for instance, the style of the definitions in Fernando's papers or in our ICASSP paper. Alejandro also did a pretty good job at making some of my definitions more concise in the graphon and transferability lectures of the GNN course.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DEFINITION %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}[$\alpha$-separated spectrum]\label{def:alpha-spectrum}
%\red{L: Here, for instance, you only have to define the set $\ccalD$. Make the definition as mathematical as possible. Any explanations of the definition can then be given in the paragraphs following it.} 
The $\alpha$-separated spectrum of a Laplace-Beltrami operator $\ccalL$ is defined as the union of the set of $\alpha$-separated eigenvalues $\ccalD$,
$$\ccalD =\{\lambda_i : i\geq 1,\ \lambda_{i}-\lambda_{i-1}>\alpha,\ \lambda_{i+1}-\lambda_i>\alpha \}$$
and the set of $\alpha$-close eigenvalues $\ccalN = \bar{\ccalD}$,
\begin{align*}
\ccalN:=\{\ccalN_1,\ccalN_2,\cdots,\ccalN_N\} \mbox{ s.t. } \min|\lambda_i-\lambda_j|>\alpha \\
\mbox{ for all } \lambda_i\in\ccalN_a, \lambda_j\in\ccalN_b, a\neq b.
\end{align*}
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \input{eigenvalues_laplacian.txt}    
    \caption{Eigenvalues of a Laplacian operator. Observe that the eigenvalues of the Laplacian operator tend to be grouped in certain parts of the spectrum.}
    \label{fig:eigenvalues_laplacian}
\end{figure}

%With Definition \ref{def:alpha-spectrum}, we can observe that all the $\alpha-$close groups and the eigenvalues in $\ccalD$ are $\alpha-$separated. In this manner, we define a filter function with frequency difference threshold $\alpha$, which we call $\alpha-$ difference threshold filter. 
% We denote the set of isolated eigenvalues as $\ccalD =\{i\geq 1:  \lambda_{i}-\lambda_{i-1}>\alpha, \lambda_{i+1}-\lambda_i>\alpha \}$ with some $\alpha>0$ predefined while $\bar\ccalD$ as its compliment. The eigenvalues in $\bar\ccalD$ can be seen as groups and within each group an eigenvalue $\lambda_i$ is close enough to its neighboring eigenvalue, i.e. $\lambda_{i}-\lambda_{i-1}\leq \alpha$. We denote that we have the group set as $\ccalN:=\{\ccalN_1,\ccalN_2,\cdots,\ccalN_N\}$. We denote the number of isolated eigenvalues and eigenvalue groups as $|\ccalD|:=D$ and $|\ccalN|:=N$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DEFINITION %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}[$\alpha$-FDT filter]\label{def:alpha-filter}
%\red{L: Here, it is not that you are applying a filter to an $\alpha$-separated spectrum; $\alpha$ is a parameter of the filter, so \textit{it is the filter which separates the spectrum.}}
On the manifold $\ccalM$, an $\alpha$-frequency difference threshold ($\alpha$-FDT) filter is a filter whose frequency response $h(\lambda)$ satisfies
\begin{equation} \label{eq:fdt-filter}
    h(\lambda)=C_n,\quad \lambda\in [\min_{i\in\ccalN_n}\lambda_i,\max_{j\in\ccalN_n}\lambda_j].
\end{equation}
for all $n=1,2,\hdots,N$. This makes the convolution operation as:
\begin{equation} \label{eqn:fdt-convolution}
\bbh(\ccalL)=\sum_{i\in \ccalD} h(\lambda_i)\langle f,\bm\phi_i\rangle \bm\phi_i +\sum_{n=1}^N C_n\langle f, E_n\rangle E_n,
\end{equation}
where $E_n$ is the eigenspace composed of $\{\bm\phi_i\}_{i\in\ccalN_n}$.
\end{definition}

{The eigenvalues $\lambda_i$ in the set $\ccalD$ are at least $\alpha$ apart from their preceding and succeeding eigenvalues $\lambda_{i-1}$ and $\lambda_{i+1}$. Hence, according to Definition \ref{def:alpha-filter}, an FDT filter with threshold $\alpha$ treats them as independent eigenvalues, like a conventional convolutional filter \eqref{eqn:filter_function} would.
The eigenvalues in the complement set $\ccalN = \bar\ccalD$ are divided in groups $\ccalN_a$ where each group contains eigenvalues that are less than $\alpha$ apart from at least one their neighbors. As such, the distance between any two groups $\ccalN_a, \ccalN_b$, $a \neq b$, is larger than $\alpha$. To achieve spectrum separation, the $\alpha$-FDT filter imposes a constant frequency response $h(\lambda_i)=C_a$ for all $i \in \ccalN_a$.} In other words, it treats all the eigenvalues in a group $\ccalN_a$ as the same. Note that, while the $h(\lambda)$ in Definition \ref{def:alpha-filter} is not a smooth function, we can still obtain a smooth approximation of an FDT filter in the form of \eqref{eqn:operator}.

%\red{This paragraph I think needs to be stressed more.}
%\green{The $\alpha$-FDT filter evaluates each eigenvalue of the spectrum. It separates the spectrum by treating all the eigenvalues within one $\alpha$-close group as the same. It forces a constant frequency response for the similar spectral components of the input signal. This is justifable because for a general continuous filter function it may also assign similar weights to the spectral components with eigenvalues that are close enough. } 
%\red{L: Here you need a paragraph to discuss Definition 3, which is one of the most important definitions of your paper. For instance, you have to explain in words what the FDT filter does --- it ``separates'' the spectrum by treating all eigenvalues in an $\alpha$-group as the same. And how does it do that? By assigning the spectral components of the input signal associated with those eigenvalues the same, constant weight $C_n$.}

\begin{figure}[t]
    \centering
    \input{filter_response.txt}    
    \caption{An $\alpha$-FDT filter that separates the spectrum of the Laplacian operator by grouping eigenvalues that are less than $\alpha$ apart in sets $\ccalN_i$. Note that the frequency response is constant for all eigenvalues in a group $\ccalN_i$.}
    \label{fig:filter-response}
\end{figure}

\subsection{FDT filter stability}
%We consider an $\alpha$-FDT filter with output $y=\bbh(\ccalL)f$ on a Riemannian manifold with Laplacian operator $\ccalL$. %\red{``The spectrum of $\ccalL$ can be represented as an $\alpha-$separated spectrum.'' L: Again, it is not that the spectrum can be represented as an $\alpha$-separated spectrum; it is the filter which achieves this.}
%With Proposition \ref{prop:finite_num}, it can be concluded that the cardinal $D:=|\ccalD|$ and $N:=|\ccalN|$ are finite. 

{Thanks to spectrum separation, $\alpha$-FDT manifold filters can be shown to be stable under the absolute perturbations to the Laplace-Beltrami operator in Definition \ref{defn:absolute_perturbations}. 
%To quantify their stability, we bound the difference between the outputs of the $\alpha$-FDT filter applied to the same input signal on the original and perturbed Laplace-Beltrami operators. 
We can state and prove this in Theorem \ref{thm:stability_filter} under Assumption \ref{ass:filter_function}.}

%Suppose that the manifold is perturbed by a symmetric operator $\bbA$, this leads to a perturbed Laplacian operator $\ccalL'=\ccalL+\bbA$ and the output $y'=\bbh(\ccalL')$. Similarly, the eigendecomposition of $\ccalL'$ is denoted as $\{\lambda'_i,\bm\phi'_i\}_{i\in\naturals}$. The stability of the manifold filter can be measured by the difference of the output signals as $\|y-y'\|$. First, we need to introduce some assumptions on the perturbation term as well as the filter function.


%\red{L: The two paragraphs above contain a lot of information that you don't have to mention anymore (e.g., instead of explaining the type of perturbation we consider, you can refer straight to Definition 1), or that you would rather mention in the theorem statement (e.g., the eigendecomposition of $\ccalL'$, if it appears at all in the statement of the theorem; if not, you can skip this definition as well). What I would do here, is that I would replace these paragraphs by something like: ``Due to spectrum separation, FDT manifold filters can be shown to be stable to absolute perturbations of the Laplace-Beltrami operator. This is stated and proved in Theorem \ref{thm:stability_filter} under Assumptions \ref{ass:perturb_norm} and \ref{ass:filter_function}.''}

%\begin{assumption}\label{ass:perturb_norm}
%The perturbation $\bbA$ [cf. Definition \ref{defn:absolute_perturbations}] is bounded as $\|A\|\leq\alpha$.
%\end{assumption}

%\red{L: Isn't it enough for $\|\bbA\|$ to be smaller than $\alpha$? I think the way it is now this assumption is problematic because the distance between two consecutive eigenvalues tends to zero with $i$, right?}

\begin{assumption}\label{ass:filter_function}
The filter function $h:\reals\rightarrow\reals$ is $B$- Lipschitz continuous and non-amplifying, i.e.,
\begin{equation}\label{eqn:filter_function}
    |h(a)-h(b)|\leq B|a-b|,\quad |h(a)|< 1.
\end{equation}
\end{assumption}

\begin{theorem}[FDT filter stability]\label{thm:stability_filter}
Let $\ccalM$ be a manifold with Laplace-Beltrami operator $\ccalL$. Let $f$ be a manifold signal and $\bbh(\ccalL)$ an $\alpha$-FDT filter on $\ccalM$ [cf. Definition \ref{def:alpha-filter}]. Consider an absolute perturbation $\ccalL'=\ccalL + \bbA$ of the Laplace-Beltrami operator $\ccalL$ [cf. Definition \ref{defn:absolute_perturbations}] where $\|\bbA\| = \epsilon \leq \alpha$. Then, under Assumption \ref{ass:filter_function} it holds
\begin{equation}\label{eqn:stability_filter}
\| \bbh(\ccalL) f -\bbh(\ccalL')f \| \leq  \frac{\pi(D+N)}{\alpha-\epsilon}\epsilon\|f\| + BD\epsilon\|f\|
\end{equation}
where $D$ and $N$ are the cardinalities of sets $\ccalD$ and $\ccalN$.
\end{theorem}

Provided that Assumption \ref{ass:filter_function} is satisfied, FDT filters are thus stable to absolute perturbations of the operator $\ccalL$. Note that this assumption is rather reasonable, as there are no constraints on the value of the Lipschitz constant $B$. The stability bound depends on (i) the variability of the FDT filter as measured by the Lipschitz constant $B$ and (ii) its frequency difference threshold, both directly through $\alpha$, and indirectly through $D$ and $N$. It is also split into two terms. The first one arises from the difference between the eigenfunctions of $\ccalL$ and $\ccalL'$, 
%which is equal to the sum of $\alpha$-separated eigenvalues and $\alpha$-close groups.%\red{L: here, describe where the first term comes from. Is it from the eigenvalues or eigenfunctions? From the separable or non-separable eigenvalues?}. 
while the second is a result of the distance between their eigenvalues.
%, which actually results from the difference of filter function combined with Assumption \ref{ass:filter_function}.}

%with a  
We observe that stability is improved if the Lipschitz constant $B$ is small. However, this causes the filter to become less discriminative and give similar response to all spectral components. With a larger $\alpha$, the FDT filter identifies fewer eigenvalues as being $\alpha$-separated, which decreases $D$. While this reflects an increase in the number of groups $N$, a certain number of eigenvalues previously in $\ccalD$ ends up being replaced by a fewer number of groups in $\ccalN$, leading $D+N$ to also decrease. Thus, larger values of $\alpha$ improve stability, but this also happens at the cost of discriminability as filters with large $\alpha$ separate the spectrum more sparsely, i.e., they identify fewer eigenvalues as being $\alpha$-separated. Interestingly, this stability-discriminability trade-off does not depend on the magnitude of the frequencies amplified by the filter (as is the case in, e.g., \cite{gama2020stability, ruiz2020graphon}). Instead, it is associated with the filter's precision in telling neighboring frequencies apart wherever they mare in the spectrum.

%becomes more stable because identifying
%separates the spectrum more sparsely, identifying fewer eigenvalues as being $\alpha$-separated, which in turn decreases $D$. Since only two eigenvalues are needed to form a new group, $D+N$ also decreases. Therefore, all of these lead to increased stability tradeoff between stability and discriminability. 

%The assumptions are general and justifiable. Assumption \ref{ass:perturb_norm} indicates that we are interested in small perturbations. With this assumption, eigenvalues of the perturbed Laplacian operator are still ordered as $0<\lambda'_1\leq \lambda'_2\leq \lambda'_3\leq \hdots$, with $\{\lambda'_i\}_{i\in\naturals^+}$ the eigenvalues of the pertrubed operator $\ccalL'$. Assumption \ref{ass:filter_function} is generic for polynomial filter functions. 

%\green{
%Theorem \ref{thm:stability_filter} indicates that by controlling the discrimination of spectral components associated with close eigenvalues, $\alpha$-FDT manifold filters can guarantee the stability with respect to absolute perturbations. Furthermore, the stability is associated with a frequency difference threshold predefined, instead of depending on the magnitude of the frequencies.}

%\red{L: Here, the first thing you have to do is discuss each and every component of the stability constant/bound (what they are, and what are the implications of the dependence on these components.) Then, you have to discuss the feasibility of the assumptions. Then, you have to discuss the implications of this theorem. What does it mean that these filters are stable? Finally, our most important conclusion is that \textit{on manifolds filter stability is associated with a frequency difference threshold, and not with the magnitude of the frequencies.}} 

%\subsection{Stability of Neural Networks on Manifold}
\subsection{Neural network stability} \label{sec:mnns}
%\green{Let $\bby=\bm\Phi(\bbH,\ccalL,f)$ be an MNN defined as \eqref{eqn:mnn} with $\alpha$-FDT filters on a Laplace-Beltrami operator $\ccalL$. With the absolute perturbation in Definition \ref{defn:absolute_perturbations} considered, we have another output as $\bby'=\bm\Phi(\bbH,\ccalL',f)$. The stability of this MNN can be measured by the difference:}
 %\begin{equation}\label{eqn:diff_MNN}
 %\|\bby - \bby'\|^2 =\sum_{k=1}^{K_L} | f_L^k - f_L^{'k}|^2.
 %\end{equation}
%  The output signal of the $l-$th layer of $\bbPhi(\bbH,\ccalL, f)$ can be written as:
%  \begin{equation}
%  f_l^k = \sigma\left( \sum_{g=1}^{K_{l-1}} \bbh_l^{kg}(\ccalL) f_{l-1}^g\right).
%  \end{equation}
%  Similarly, for the perturbed Laplacian operator $\ccalL'$ the corresponding neural network is $\bbPhi(\bbH',\ccalL',f)$ the output signal can be written as:
%  \begin{equation}
%  f_l^{'k} = \sigma\left( \sum_{g=1}^{K_{l-1}} \bbh_l^{kg}(\ccalL') f_{l-1}^{'g}\right).
%  \end{equation}
Manifold neural networks with banks of filters like the one in \eqref{eq:fdt-filter} inherit the stability properties of $\alpha$-FDT filters. This is demonstrated in Theorem \ref{thm:stability_nn} under Assumption \ref{ass:activation}.

\begin{assumption}\label{ass:activation}
 The activation function $\sigma$ is normalized Lipschitz continous, i.e., $|\sigma(a)-\sigma(b)|\leq |a-b|$, with $\sigma(0)=0$.
\end{assumption}
 
 %\red{L: Rewrite the statement of this theorem in the image of Theorem 1.}
\begin{theorem}[Neural network stability]\label{thm:stability_nn}
 Let $\ccalM$ be a manifold with Laplace-Beltrami operator $\ccalL$. Let $f$ be a manifold signal and $\bm\Phi(\bbH,\ccalL,f)$ an $L$-layer manifold neural network on $\ccalM$ \eqref{eqn:mnn} with $F_0=F_L=1$ input and output features and $F_l=F,i=1,2,\hdots,L-1$ features per layer, and where the filters $\bbh(\ccalL)$ are $\alpha$-FDT filters [cf. Definition \ref{def:alpha-filter}]. 
 Consider an absolute perturbation $\ccalL'=\ccalL + \bbA$ of the Laplace-Beltrami operator $\ccalL$ [cf. Definition \ref{defn:absolute_perturbations}] where $\|\bbA\| = \epsilon \leq \alpha$. 
 %With the given manifold neural network architecture [cf. \eqref{eqn:mnn}], we have $\bby=\bm\Phi(\bbH,\ccalL,f)$ and $\bby'=\bm\Phi(\bbH,\ccalL',f)$ with $L$ layers. With the number of filters on each layer set as 
 Then, under Assumptions \ref{ass:filter_function} and \ref{ass:activation} it holds:
 \begin{align}\label{eqn:stability_nn}
 \begin{split}
    \|\bm\Phi(\bbH,\ccalL,f)-&\bm\Phi(\bbH,\ccalL',f)\| \\
    &\leq LF^{L-1}\left(\frac{\pi(D+N)}{\alpha-\epsilon}+BD\right)\epsilon \|f\|.
\end{split}
 \end{align}
where $D$ and $N$ are the cardinalities of sets $\ccalD$ and $\ccalN$.
 \end{theorem}
 
Deep neural networks on manifolds are thus also stable to absolute perturbations provided that the activation function is normalized Lipschitz. This assumption is satisfied by most common activation functions, such as the ReLU, the modulus function and the sigmoid. Here, the same general comments as in the case of Theorem \ref{thm:stability_filter} hold, with the difference that in Theorem \ref{thm:stability_nn} the stability bound also depends on the number of layers $L$ and the number of features per layer $F$ of the MNN.

%\red{L: I don't think you need this paragraph below, because we are already saying this in the intro. If you want to reinforce what we said in the intro, you can say something like what is said in the second paragraph there --- because manifolds are models for graphs (or g) we can expect this stability result to extend to GNNs on graphs sampled from manifolds; and that a formal stability analysis on these graphs would rely on a CNN transferability analysis from manifolds to graphs.}

{As graphs can be seen as discretizations of manifolds, therefore we can use graph neural networks to realize the function of manifold neural networks. Combined with the transferability analysis from manifolds to graphs, we could state that the stability result that we have in Theorem \ref{thm:stability_nn} can be extended to graph neural networks.}
%\red{Comment that, in practice, this result is actually a stability result for GNNs.}
 
 



==> stability of NN on Rie-manifolds-eusipco/intro.tex <==

Convolutional neural networks (CNNs) are machine learning architectures made up of layers where each layer composes a bank of convolutional filters with a pointwise nonlinearity. On problems where data is Euclidean, they have become a popular architecture due to their impressive performance in tasks ranging from speech recognition \cite{han2020contextnet} to computer vision \cite{gustafsson2020evaluating}, which is largely attributed to the fact that CNNs are provably stable \cite{bruna2013invariant}. %CNNs have become a popular architecture in problems where data is Euclidean. 
But in the physical world, their application is limited because many problems deal with data that is non-Euclidean. This is the case, for instance, of resource allocation in wireless ad-hoc communication networks \cite{wang2020unsupervised}, detection and recognition in social networks \cite{nguyen2017robust} and prediction of influenza epidemic outbreaks \cite{wang2019defsi}. 

%As a result, there has been an increasing interest in extending deep convolutional neural network architectures to non-Euclidean domains such as graphs and manifolds. 

In recent years, a myriad of extensions of CNNs to non-Euclidean domains have been proposed to fill that gap \cite{bronstein2017geometric,gama2019convolutional, scarselli2008graph, defferrard2020deepsphere}.
These architectures have been able to reproduce the successes of CNNs on Euclidean domains to a large extent \cite{xu2018powerful, wu2020comprehensive}, which naturally sparks the question of whether non-Euclidean CNNs are also stable. In this paper, we aim to answer this question by analyzing the properties of CNNs defined on the most general type of non-Euclidean domain --- the manifold. By focusing on manifolds, our analysis has the benefit of being broad enough so that it can also be particularized to more specific non-Euclidean domains such as graphs, which can be seen as manifold discretizations. 
%Given that graphs can be seen as a discretizations of manifolds, our analysis is broad enough to encompass 
%by analyzing the properties of CNNs defined on Riemannian manifolds.

Explicitly, we study the stability of manifold CNNs to absolute perturbations of the Laplace-Beltrami operator $\ccalL$ associated with the manifold (Definition \ref{defn:absolute_perturbations}). We start by analyzing the stability of the convolution operation, which is defined as a pointwise operation on the spectrum of $\ccalL$. Given that absolute perturbations of $\ccalL$ spawn absolute perturbations to all of its eigenvalues, designing stable manifold convolutions is challenging because the spectrum of the Laplace-Beltrami operator is infinite-dimensional. We address this challenge by introducing frequency difference threshold (FDT) filters (Definition \ref{def:alpha-filter}), which separate the Laplacian spectrum into groups of eigenvalues that are less than some threshold $\alpha$ apart. We then show that these filters are stable to absolute perturbations of $\ccalL$ (Theorem \ref{thm:stability_filter}), and that this property is inherited by manifold CNNs (Theorem \ref{thm:stability_nn}). The main implication of these results is that there is a trade-off between the stability and discriminability of manifold neural networks in the form of the frequency difference threshold of the FDT filters.

Related work includes a comprehensive study of the stability of graph neural networks (GNNs) in \cite{gama2019stability} and \cite{gama2020stability}, which consider absolute and relative perturbations of the graph structure respectively, and the GNN stability analysis in \cite{zou2020graph}, which focuses on perturbations of the graph spectrum.
More in line with our paper, \cite{ruiz2020graph} studies stability of GNNs to perturbations of the underlying graph model, which is assumed to be a graphon. Unlike manifolds, however, graphons can only model dense graphs. 
More flexible models such as continuous graph models with tunable sparsity and generic topological spaces have been considered in \cite{keriven2020convergence} and \cite{levie2019transferability} respectively, but these papers focus on the transferability and not on the stability of convolutional neural networks in these domains.
%\red{Cite ICASSP, explain why what we do is different and more generic. Then cite transferability papers.}


%This transferability property also builds a connection between neural networks on graphs and the ones on manifolds. \cite{ruiz2020graph} is the most in line with our paper, instead that it focuses on the graphon instead of a general topological space. We include the general perturbations to the underlying manifold.

%Transferability, i.e., the ability to transfer machine learning architectures between different supports, is also the object of papers which rely on the definition convolutional architectures on graph models such as graphons \cite{X} and generic topological spaces.

%graph neural networks (GNNs) have recently become , in particular has been widely studied recently. The difference mainly lies in that signals are now defined over the nodes on graph or manifold domains. The convolution filters can be replaced by a linear operator on Laplacian of graphs or manifolds. With the assumption that the Laplacian is known as the structure, the linear operator can be learned to get a suitable representation. 
%Since the success of CNNs has been seen in many fields, there has been an increasing interest in understanding the underlying working principles and properties.
%In practice, physical noise and uncertainties lead to perturbation of the underlying manifolds. The outputs may differ because of this perturbed input structure. The perturbation usually comes from measurement noise. This can be interpreted physically as the fault detection and uncertain feedbacks. This leads to the necessity of the stability analysis with a perturbed underlying structure. \cite{bruna2013invariant} studies the invariance of scattering convolutional networks. Similarly in GNNs,  \cite{keriven2020convergence} and \cite{ruiz2020graph} study the stability of convergent graph sequences. 

%In our work, we focus on neural networks on Riemannian manifolds. 
The rest of this paper is organized as follows. We start with a brief review of manifolds and Laplacian operators in Section \ref{sec:prelim}. We further introduce the framework of manifold convolutions and neural networks. In Section \ref{sec:filters}, we introduce FDT filters and prove that the filters are stable under absolute perturbations of the Laplacian operator. We then extend this analysis to neural networks. Our results are verified numerically on a power allocation problem in wireless adhoc networks in Section \ref{sec:sims}, and conclusions are presented in Section \ref{sec:conclusions}.



==> stability of NN on Rie-manifolds-eusipco/mySections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\bf #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> stability of NN on Rie-manifolds-eusipco/prelims.tex <==
%!TEX root = conference-stability.tex
In order to analyze the stability properties of neural networks on manifolds, we start by reviewing the notions of signals, Laplacian operators and convolutional neural networks in these domains.

%%%%%%%%%%%%%%%%
%% Subsection %%
%%%%%%%%%%%%%%%%
\subsection{Manifolds and manifold signals}
{A manifold is a topological space that is locally Euclidean around each point. More formally, a differentiable $d$-dimensional manifold is a topological space where each point has a neighborhood that is homeomorphic to a $d$-dimensional Euclidean space, i.e., the tangent space.} A Riemannian manifold, denoted $(\ccalM,g)$, is a real and smooth manifold $\ccalM$ equipped with a positive definite inner product $g_x$ on the tangent space $T_x\ccalM$ at each point $x$. The collection of tangent spaces of all points on $(\ccalM, g)$ is denoted as $T\ccalM$, and the collection  %\red{(L: Hilbert spaces? Aren't these the spaces of $L^2$ functions or, equivalently, square integrable functions?)}
of scalar functions and tangent vector functions on $(\ccalM,g)$ are denoted as $L^2(\ccalM)$ and $L^2(T\ccalM)$ respectively. In this paper, we consider compact Riemannian manifolds $\ccalM$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{manifold-eps-converted-to.pdf}
    \caption{An example of manifold signal where the curve is the underlying manifold structure. Colors stand for values of the signal at the point.}
    \label{fig:manifold}
\end{figure}
Data supported on the manifold $\ccalM$ is represented as manifold signals, which are defined as functions $f\in L^2(\ccalM)$.
%\red{L: Add the definition of a general manifold before introducing Riemannian manifolds here. It would be helpful to explain manifolds in words, or to provide a visual interpretation of them as well. If possible, mention the dimension of the manifold here ($d$).}
%\red{L: Zhiyang, can you include a picture of a manifold with colors indicating the values of a manifold signal?}
Given a manifold signal $f\in L^2(\ccalM):\ccalM\rightarrow \reals$, the Laplace-Beltrami operator $\ccalL$ is defined as
\begin{equation}\label{eqn:Laplacian}
    \ccalL f=-\text{div}(\nabla f),
\end{equation}
where $\nabla: L^2(\ccalM)\rightarrow L^2(T\ccalM)$ is an operator called \emph{intrinsic gradient}. Compared with the classical notion of gradient, which indicates the direction of the fastest change of a function at a given point, the difference here is that the direction indicated by the intrinsic gradient is a tangent vector in $L^2(T\ccalM)$. The operator $\text{div}$ %\red{(L: Never start a sentence with a symbol.)} 
is the \emph{intrinsic divergence}, which is adjoint to the gradient operator. Akin to the Laplacian operator in Euclidean domains or the graph Laplacian in graph signal processing (GSP), the Laplace-Beltrami operator defines a notion of shift for signals on a manifold $\ccalM$. In fact, $\ccalL$ has a similar interpretation to that of the graph Laplacian as the difference between the local average function value around a point and the function value at the point itself \cite{bronstein2017geometric}. 
%It is widely used in signal processing and learning techniques on topological spaces due to its well-performed eigenfunction, which could be generalized as eigenbasis for spectral analysis on manifolds\cite{bronstein2017geometric}.

The Laplacian operator $\ccalL$ is a self-adjoint and positive-semidefinite operator. As such, it admits an eigendecomposition given by
\begin{equation} \label{eqn:Laplacian-spectrum}
    \ccalL f=\sum_{i=1}^\infty \lambda_i\langle f, \bm\phi_i \rangle \bm\phi_i.
\end{equation}
where $\lambda_i$ are real eigenvalues and $\bm\phi_i$ are the corresponding eigenfunctions. Because the manifold $\ccalM$ is compact, the spectrum $\{\lambda_i,\bm\phi_i\}_{i\in\naturals^+}$ is additionally discrete. {If the eigenvalues are ordered in increasing order as $0<\lambda_1\leq \lambda_2\leq\lambda_3\leq \hdots$, it can be shown that, for a manifold on $d$ dimensions, $\lambda_i$ grows as $i^{2/d}$ \cite{arendt2009weyl}. 

Similarly to how the eigenvalues of the graph Laplacian are interpreted as frequencies in GSP, we interpret the Laplacian-Beltrami operator eigenvalues $\lambda_i$ as frequencies associated with oscillation modes $\bm\phi_i$.
Moreover, since the eigenfunctions $\bm\phi_1,\bm\phi_2,\hdots$ form an orthonormal basis of $L^2(\ccalM)$, a change of basis operation for signals $f$ can be defined, i.e., manifold signals $f\in L^2(\ccalM)$ can be represented on the manifold's eigenbasis as $f=\sum_{i=1}^\infty \langle f, \bm\phi_i \rangle \bm\phi_i$.}

%%%%%%%%%%%%%%%%
%% Subsection %%
%%%%%%%%%%%%%%%%
\subsection{Manifold convolutions and manifold neural networks}

Drawing a parallel with the spectral convolution operation on Euclidean domains, we leverage the eigendecomposition of the Laplacian \eqref{eqn:Laplacian-spectrum} to define the convolution of manifold signals as a pointwise operation in the spectrum of $\ccalL$. Explicitly, we define a manifold convolutional filter \bbh(\ccalL) as
\begin{equation}\label{eqn:operator}
\bbh(\ccalL) f:=\sum_{i=1}^\infty \sum_{k=0}^{K-1} h_k \lambda_i^k \langle f,\bm\phi_i \rangle \bm\phi_i
\end{equation}
where $h_0, \ldots, h_{K-1}$ are the filter coefficients or taps.

Projecting $\bbh(\ccalL)f$ onto $\{\bm\phi_i\}_{i \in \naturals^+}$, we see that the spectral response of the manifold convolution is is given by $h(\lambda) = \sum_{k=0}^{K-1} h_k \lambda^k$. This highlights the fact that the frequency response of a manifold convolution only depends on the coefficients $h_k$ and the eigenvalues of the Laplace-Beltrami operator. It also implies that, if the underlying manifold changes --- and thus $\ccalL$ ---, the behavior of the filter $\bbh$ can be replicated on the new manifold $\ccalM'$ by evaluating $h(\lambda)$ at the eigenvalues of the new Laplacian $\ccalL'$. Another important consequence of the spectral representation of $\bbh(\ccalL)$ being a polynomial is that, as $K \to \infty$, $\bbh(\ccalL)$ can be used to implement any smooth spectral response $h(\lambda)$ with convergent Taylor series around each $\lambda_0 \in \reals$ as $K \to \infty$ \cite{smyth2014polynomial}.

%When considering a $d$-dimensional Riemannian manifold $\ccalM$ with the Laplace-Beltrami operator denoted as $\ccalL$. Functional calculus is often implemented for spectral convolution operation to overcome the non-transferability and high computational complexity. When applying functions $h:\reals \rightarrow \reals$ on operators in $L^2(\ccalM)$. The result can be written as:
%\begin{equation}\label{eqn:operator}
%\bbh(\ccalL) f:=\sum_i h(\lambda_i) \langle f,\bm\phi_i \rangle \bm\phi_i,
%\end{equation}
%where $\{\lambda_i,\bm\phi_i\}_{i\in\naturals^+}$ is the eigendecomposition of the operator $\ccalL$ with $\lambda_i$ as eigenvalues and $\bm\phi_i$ as the corresponding eigenfunctions.
%The eigenvalues are ordered as $0<\lambda_1\leq \lambda_2\leq\lambda_3\leq \hdots$ in an increasing order. As the index $i$ goes to infinity, the eigenvalue grows with the order of $i^{2/d}$ with $d$ as the dimension of the manifold\cite{arendt2009weyl}.

%\red{(L: ``Deep Neural Networks are widely used to build a mapping from an input signal to a target representation.'' Please remove this sentence. This type of sentence is too vague, and not necessary in the preliminary section. It will usually be in the introduction.)}
From the definition of the convolution operation on $\ccalM$ \eqref{eqn:operator}, convolutional neural networks (CNNs) are straightforward to define. A CNN consists of a cascade of $L$ layers, each of which contains a bank of convolutional filters followed by a nonlinear activation function. Denoting the nonlinearity $\sigma$, the $l$-th layer of a $L$-layer CNN on the manifold $\ccalM$ is given by:
%At each layer, a bank of filters is applied to the output features of the previous layer followed by a nonlinear activation function. Iteratively, the output of the last layer can be seen as the final estimated representation. 
%\red{(L:``The convolution operation on Laplacian operators defined in \eqref{eqn:operator} is a filter based on the Riemannian manifold. Therefore, we can use this as filters on each layer. With the same architecture, deep neural networks on manifold can be obtained as:'' Please remove these sentences. You don't have to justify a definition. You simply introduce it.)}
\begin{equation}\label{eqn:mnn}
f_l^p(x) = \sigma\left( \sum_{q=1}^{F_{l-1}} \bbh_l^{pq}(\ccalL) f_{l-1}^q(x)\right)
\end{equation}
for $l=1,2,\hdots,L$. Each of the filters $\bbh_l^{pq}(\ccalL)$ is as in \eqref{eqn:operator} and maps the $q$-th feature from the $l-1$-th layer to the $p$-th feature of the $l$-th layer for $1\leq q\leq F_{l-1}$ and $1\leq p\leq F_{l}$. The output of this neural network is given by $y^p = f_L^p$ for $1 \leq p \leq F_L$ and the input features at the first layer, $f_0^q$, are the input data $f^q$ for $1\leq q\leq F_0$. For a more concise representation of this CNN, we can alternatively write it as the map $\bby = \bbPhi(\bbH,\ccalL, f)$, where $\bbH$ is a tensor gathering the learnable parameters $\bbh_l^{pq}$ at all layers of the CNN. We will refer to this map as a manifold convolutional neural network or manifold neural network (MNN) for short.



==> stability of NN on Rie-manifolds-eusipco/proof.tex <==
\section{Proof of Theorem \ref{thm:stability_filter}}
\begin{proof}
Begin with the definition of spectral convolution operators in \eqref{eqn:operator}, we can rewrite the norm difference between two outputs as:
\begin{align}
   \nonumber & \left\| H(\ccalL) f  - H(\ccalL+A)f\right\|
    \\
  \nonumber  & = \| \sum_{i\in\ccalD} h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i +\sum_{n\in\ccalN} h_n \langle f, E_n  \rangle E_n \\
    & - \sum_{i\in\ccalD} h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i  -\sum_{n\in\ccalN} h_n \langle f, E'_n  \rangle E'_n \| 
  \\ \nonumber & \leq  \left\| \sum_{i\in \ccalD} h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i  - \sum_{i\in \ccalD} h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i \right\| \\
  & + \sum_{n\in\ccalN}\|h_n\| \left\|  \langle f, E_n  \rangle E_n -   \langle f, E'_n  \rangle E'_n  \right\|  \label{eqn:HS}
  % &\leq \left\| \sum_{n\in \ccalD_1} h(\lambda_{n}) \langle f, \bm\phi_n \rangle \bm\phi_n -  h(\lambda'_{n}) \langle f, \bm\phi'_n \rangle \bm\phi'_n \right\| + \left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -  \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} \right\| 
    %\\
    %&\leq \left\| \sum_{n\in \ccalD_1} h(\lambda_{n}) \langle f, \bm\phi_n \rangle \bm\phi_n -  h(\lambda'_{n}) \langle f, \bm\phi'_n \rangle \bm\phi'_n \right\| + \{\|h(E_{\bar\ccalD_1})\|,\|h(E'_{\overline{\ccalD}})\|\} \|\langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} - \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} \| 
\end{align}
%The decomposition in \eqref{eqn:decompose} results from the boundedness of filter function. 
$E_{n}$ is column space of eigenfunctions $[\bm\phi_i]_{i\in\ccalN_n}$ while $E'_{n}$ is column space of eigenfunctions $[\bm\phi'_i]_{i\in\ccalN_n}$.

For the first term in \eqref{eqn:HS}, with the triangle inequality the norm difference can then be written as:
\begin{align}
 & \nonumber \left\| \sum_{i\in \ccalD} h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i  -  h(\lambda'_i )  \langle f, \bm\phi'_i \rangle \bm\phi'_i \right\| \\
 & =\|\sum_{i \in \ccalD}  h(\lambda_{i}) \langle f, \bm\phi_i \rangle \bm\phi_i -  h(\lambda_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i +  h(\lambda_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i\nonumber \\
  & \qquad \qquad \qquad \qquad \qquad \qquad\qquad \quad- h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i \| \\
 &\nonumber \leq \left\|\sum_{i \in \ccalD_1}  h(\lambda_i  \langle f, \bm\phi_i \rangle \bm\phi_i -  h(\lambda_i ) \langle f, \bm\phi'_i \rangle \bm\phi'_i\right\|\\
 & \qquad \qquad \quad+ \left\|\sum_{i \in \ccalD_1} h(\lambda_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i -  h(\lambda'_{i}) \langle f, \bm\phi'_i \rangle \bm\phi'_i \right\|\\
 &\leq \left\| \sum_{i \in \ccalD_1}  h(\lambda_i)\left( \langle f, \bm\phi_i \rangle\bm\phi_i-\langle f, \bm\phi_i \rangle\bm\phi'_i +\langle f, \bm\phi_i \rangle\bm\phi'_i - \langle f, \bm\phi'_i \rangle \bm\phi'_i \right) \right\| \nonumber \\
 & \qquad \qquad \qquad\qquad+ \left\|\sum_{i \in \ccalD_1}  (h(\lambda_i ) -h(\lambda'_i)  \langle f, \bm\phi'_i \rangle \bm\phi'_i  \right\| \\
 & \leq \left\| \sum_{i \in \ccalD_1} h(\lambda_i )\langle f, \bm\phi_i \rangle (\bm\phi_i - \bm\phi'_i ) \right\| +\left\|  \sum_{i \in \ccalD_1}  h(\lambda_i )\langle f, \bm\phi_i - \bm\phi'_i  \rangle \bm\phi'_i \right\|\nonumber \\ 
 &\qquad \qquad \qquad\qquad + \left\|\sum_{i \in \ccalD_1}  (h(\lambda_i ) -h(\lambda'_i) ) \langle f, \bm\phi'_i \rangle \bm\phi'_i  \right\|\label{eqn:3}
    % \\
    % &\leq 2\sum_{n }  \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| + \sum_{n }  \left\|h(\lambda_{n}) -h(\lambda'_n) \right\|  \left\| f \right\| 
    % &\left\| \sum_{n\in C} h(\lambda_n)\langle f, \bm\phi_n \rangle (\bm\phi_n-\bm\phi'_n) \right\| +\left\|  \sum_{n\in C}   h(\lambda_n)\langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\|+ \left\|\sum_{n\in C}   (h(\lambda_{n}) -h(\lambda'_n) ) \langle f, \bm\phi'_n \rangle \bm\phi'_n  \right\|
    \\
 &\leq 2 \sum_{i \in \ccalD_1}    \left\|h(\lambda_i )\right\| \left\|f\right\| \left\|\bm\phi_i-\bm\phi'_i \right\| + \sum_{i \in \ccalD_1}   \left\| (h(\lambda_i ) -h(\lambda'_i ) )\right\|\|f\| \label{eqn:2}
\end{align}

For the second term in \eqref{eqn:HS}, similarly with the triangle inequality, we have:
\begin{align}
\sum_{n\in\ccalN}\|h_n\| \left\|  \langle f, E_n  \rangle E_n -   \langle f, E'_n  \rangle E'_n  \right\| \leq 2\sum_{n\in\ccalN} \|E_n-E'_n\|
\end{align}
%\begin{align}
%&\left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -  \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} \right\| \\ 
%&\leq \left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -   \underline{h}(E'_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} +  \underline{h}(E'_{\bar\ccalD_1}) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} - \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1}   \right\| \\ 
%& \leq \left\| \overline{h}(E_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1} -   \underline{h}(E'_{\bar\ccalD_1}) \langle f, E_{\bar\ccalD_1} \rangle E_{\bar\ccalD_1}\right\| + \left\|   \underline{h}(E'_{\bar\ccalD_1}) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1} - \underline{h}(E'_{\bar\ccalD_1} ) \langle f, E'_{\bar\ccalD_1} \rangle E'_{\bar\ccalD_1}   \right\| \\
%& \leq \left\|  \overline{h}(E_{\bar\ccalD_1}) -  \underline{h}(E'_{\bar\ccalD_1}) \right\| \|f\| + 2\left\| E_{\bar\ccalD_1} - E'_{\bar\ccalD_1}  \right\|\|f\| \\
%&\leq 2\left\| E_{\bar\ccalD_1} - E'_{\bar\ccalD_1}  \right\|\|f\|
%\end{align}

% The first and second terms can be analyzed separately in two parts. We design the operator in the form that $h(\lambda_n)$ is constant for $\lambda_n>c$. Therefore it can be rewritten as:
% \begin{align}
% &\left\| \sum_{n } h(\lambda_n)\langle f, \bm\phi_n \rangle (\bm\phi_n-\bm\phi'_n) \right\| +\left\|  \sum_{n }  h(\lambda_n)\langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\| \\
% &\leq \left\| \sum_{n=1 }^\bbarM h(\lambda_n)\| f\| \|\bm\phi_n\|   (\bm\phi_n-\bm\phi'_n) \right\| + \left\| \sum_{n=\bbarM+1}^\infty h(\lambda_n)\|f\| \|\bm\phi_n\| (\bm\phi_n-\bm\phi'_n) \right\| + \nonumber\\
% &\qquad \qquad \qquad \qquad\qquad \qquad\left\|  \sum_{n=1 }^\bbarM h(\lambda_n)\|f\| \|\bm\phi_n-\bm\phi'_n \| \bm\phi'_n \right\|+\left\|  \sum_{n=\bbarM+1 }^\infty  h(\lambda_n)\langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\|  \\
% &\leq 2 \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| +\left\| h(\lambda) \|f\|\sum_{n=\bbarM+1}^\infty(\bm\phi_n-\bm\phi'_n) \right\| + \left\| h(\lambda)\sum_{n=\bbarM+1}^\infty \langle f, \bm\phi_n-\bm\phi'_n \rangle \bm\phi'_n \right\|\\
% & \leq 2 \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| + \|h(\lambda)\|\|f\| \left\|\sum_{n=\bbarM+1}^\infty (\bm\phi_n-\bm\phi'_n)\right\| + \|h(\lambda)\| \sum_{n=\bbarM+1}^\infty \langle f, \bm\phi_n-\bm\phi'_n \rangle 
% \label{eqn:1}\\
% & \leq 2 \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| +  2\|h(\lambda)\|\|f\|
% \left\|\sum_{n=\bbarM+1}^\infty (\bm\phi_n-\bm\phi'_n)\right\|.
% \label{eqn:2}
% \end{align}
% From \eqref{eqn:1} to \eqref{eqn:2}, this is due to the linearity of inner products. 

% By grouping eigenvalues that are close enough, i.e. $ \ccalC = \{ i\leq \bbarM: \min\{ |\lambda_i-\lambda'_{i+1}|, |\lambda_i-\lambda'_{i-1}|, |\lambda'_i-\lambda_{i+1}|, |\lambda'_i-\lambda_{i-1}| \} > \delta \} $, we can decompose the first item as:
% \begin{align}
%     \sum_{n=1 }^\bbarM   \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\|= \sum_{n\in \ccalC} \left\|h(\lambda_n)\right\| \left\|f\right\| \left\|\bm\phi_n-\bm\phi'_n\right\| + \max\limits_{i\in \bar\ccalC} \left\|h(\lambda_i)\right\|\left\|f\right\| \left\| E_{\bar\ccalC}  -E'_{\bar\ccalC}\right\|
% \end{align}
Now we need to include two important lemmas to analyze the influence on eigenvalues and eigenspaces caused by the perturbation.
\begin{lemma}\label{lem:eigenvalue_absolute}[Weyl's Theorem]
The eigenvalues of operators $\ccalL$ and $\ccalL'$ satisfy:
\begin{equation}
|\lambda_n-\lambda'_n|\leq \|\bbA\|\leq \epsilon.
\end{equation}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:eigenvalue_absolute}]
First assume that $\ccalL$ and $\bbA$ are symmetric operators. Let $\lambda_1\leq \lambda_2\leq \dots\leq \lambda_n\leq \cdots$ be the eigenvalues arranged in the ascending order. For each subspace $T$ of the manifold, define:
\begin{align}
    \lambda[\ccalL, T] =\min_{u\in T, \|u\|=1} \langle \ccalL, u \rangle.
\end{align}
The minimax principle asserts that:
\begin{align}
    \lambda_n(\ccalL)=\max_{codim T = n-1}\lambda[\ccalL, T]=\max_{codim \leq n-1} \lambda[\ccalL, T].
\end{align}
Each $u$ has the expansion:
\begin{align}
    u=\sum \xi_n\bm\phi_n, \quad \|u\|^2=\sum |\xi_n|^2.
\end{align}
Then:
\begin{align}
    \ccalL u=\sum \xi_n \ccalL \bm\phi_n,\quad \langle \ccalL u,u \rangle =\sum \lambda_n(\ccalL) |\xi_n|^2.
\end{align}
Therefore,
\begin{align}
    \lambda_1(\ccalL) \leq  \frac{\langle \ccalL u, u\rangle }{\|u\|^2} \leq \max_n\lambda_n(\ccalL).
\end{align}
Then for any $1\leq k $, we have:
\begin{align}
    \lambda_k(\ccalL+ \bbA) &=\max_{codim T\leq n-1} \min_{ u\in T, \|u\|=1}  \langle (\ccalL + \bbA) u, u\rangle \\
    & = \max_{codim T\leq n-1} \min_{ u\in T, \|u\|=1} \left \langle  \ccalL  u, u\rangle + \langle \bbA u, u\rangle   \right)\\
    & \geq \max_{codim T\leq n-1} \min_{  u\in T, \|u\|=1}  \left\langle  \ccalL  u, u\rangle   + \lambda_1(\bbA) \right)\\
    & = \lambda_1(\bbA)+ \max_{codim T\leq n-1} \min_{  u\in T, \|u\|=1 } \langle  \ccalL  u, u\rangle  \\
    & = \lambda_k(\ccalL)+\lambda_1(\bbA).
\end{align}
Similarly, we can have $\lambda_k(\ccalL+ \bbA) \leq \lambda_k(\ccalL)+ \max_n\lambda_n(\bbA)$. This leads to $\lambda_1(\bbA)\leq \lambda_k(\ccalL + \bbA )-\lambda_k(\ccalL) \leq \max_n\lambda_n(\bbA)$.
\end{proof}

To measure the difference of eigenspaces, 
\begin{lemma}[Davis-Kahan $\sin\theta$ Theorem]\label{lem:davis-kahan}
Suppose the spectra of $\ccalL$ and $\ccalL'$ are partitioned as $\sigma\bigcup\Sigma$ and $\omega\bigcup \Omega$ respectively, with $\sigma\bigcap \Sigma=\emptyset$ and $\omega\bigcap\Omega=\emptyset$. Then we have:
\begin{equation}
\|E_\ccalL(\sigma)-E_{\ccalL'}(\omega)\|\leq \frac{\pi}{2}\frac{\|(\ccalL'-\ccalL)E_\ccalL(\sigma)\|}{d}\leq \frac{\pi}{2}\frac{\|(\ccalL'-\ccalL)\|}{d},
\end{equation}
where $d$ satisfies: $\min_{x\in\sigma,y\in\Omega}|x-y|\geq d$ and $\min_{x\in\Sigma,y\in\omega}|x-y|\geq d$.
\end{lemma}


For the first term in \eqref{eqn:2}, we employ Lemma \ref{lem:davis-kahan} and therefore we have $\sigma=\lambda_n$ and $\omega=\lambda'_n$, for $n\in C$ we can have: 
\begin{align}
\left\| \bm\phi_n -\bm\phi'_n\right\| \leq \frac{\pi}{2} \frac{\|\bbA\|}{\delta}.
\end{align}

Similarly, for the second term in \eqref{eqn:HS} we have $\sigma=\{\lambda_i\}_{i\in\ccalN_n}$ and $\omega=\{\lambda'_i\}_{i\in\ccalN_n}$, 
\begin{align}
\left\| E_{n}  -E'_{n}\right\| \leq \frac{\pi}{2} \frac{\|\bbA\|}{\delta}.
\end{align}

The second term in \eqref{eqn:2} can be bounded by the Lipschitz continuity of $h$ combined with Lemma \ref{lem:eigenvalue_absolute}:
\begin{align}
\|\sum_{i\in\ccalD }   (h(\lambda_{i}) -& h(\lambda'_i) ) \langle f, \bm\phi'_i \rangle \bm\phi'_i  \| \nonumber\\
&\leq \sum_{i\in\ccalD}\left\| (h(\lambda_{i}) -h(\lambda'_i) )\right\|\|f\| \\
&\leq \sum_{i\in\ccalD} C |\lambda_i - \lambda'_i |\|f\|\leq |\ccalD| C \epsilon\|f\|.
\end{align}

%For $h(\lambda_n)$ is a constant for $n>\bbarM$, we can construct this by summing the bandwidth-limited filter for $n\leq \bbarM$ and a low-pass filter $g(\lambda)$ with $g(\lambda_n)$  a constant for $n>\bbarM$ and 0 otherwise. The low-pass filter is stable because it can be seen as the sum of a constant filter and a high-pass filter with an opposite value. 
\end{proof}

\section{Proof of Theorem \ref{thm:stability_nn}}
The difference can therefore be written as:
 \begin{align}
 &\nonumber\| f_l^k - f_l^{'k} \|=\\
 &\left\|  \sigma\left( \sum_{g=1}^{K_{l-1}} H_l^{kg}(\ccalL) f_{l-1}^g\right) -  \sigma\left( \sum_{g=1}^{K_{l-1}} H_l^{'kg}(\ccalL') f_{l-1}^{'g}\right) \right\|.   
 \end{align}
 With the assumption that $\sigma$ is normalized Lipschitz, we have:
 \begin{align}
  \| f_l^k - f_l^{'k} \| &\leq \left\| \sum_{g=1}^{K_{l-1}}  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g}  \right\|\\
  &\leq \sum_{g=1}^{K_{l-1}} \left\|  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g} \right\|.
 \end{align}
 By adding and subtracting $H_l^{'kg}(\ccalL') f_{l-1}^{g}$ from each term, combined with the triangle inequality we can get:
 \begin{align}
 &\left\|  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g} \right\| \\
 &\leq \left\|  H_l^{kg}(\ccalL) f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{g} \right\| \\
 &+ \left\| H_l^{'kg}(\ccalL') f_{l-1}^g - H_l^{'kg}(\ccalL') f_{l-1}^{'g} \right\|.
 \end{align}
 The first term can be bounded with \eqref{eqn:stability_filter}. The second term can be decomposed by Cauchy-Schwartz inequality and bound for filter function as:
 \begin{align}
 \| f_{l}^k - f_l^{'k} \| \leq \sum_{g=1}^{K_{l-1}} C_{per} \epsilon \bbarM \| f_{l-1}^g\| + \sum_{g=1}^{K_{l-1}} \| f_{l-1}^g - f_{l-1}^{'g} \|.
 \end{align}
 To solve this recursion, we need to compute the bound for $\|f_l^k\|$. By the Lipschitz continuity of $\sigma$ and the fact that $\sigma(0)=0$, we can get:
 \begin{align}
 \| f_l^k \|&\leq \left\| \sum_{g=1}^{K_{l-1}} H_l^{kg}(\ccalL) f_{l-1}^{g}  \right\|\leq  \sum_{g=1}^{K_{l-1}}  \left\| H_l^{kg}(\ccalL)\right\|  \|f_{l-1}^{g}  \| 
 \\ &\leq   \sum_{g=1}^{K_{l-1}}   \|f_{l-1}^{g}  \| \leq \prod\limits_{l'=1}^{l-1} K_{l'} \sum_{g=1}^{K_0}\| f^g \|.
 \end{align}
 Insert this conclusion back to solve the recursion, we can get:
 \begin{align}
 \| f_{l}^k - f_l^{'k} \|\leq l C_{per}\epsilon \left( \prod\limits_{l'=1}^{l-1} K_{l'} \right) \sum_{g=1}^{K_0} \|f^g\|.
 \end{align}
 Replace $l$ with $L$ we can obtain:
 \begin{align}
 \|y-y'\|^2 \leq \sum_{f=1}^{K_L} \left( L C_{per}\epsilon \left( \prod\limits_{l'=1}^{L-1} K_{l'} \right) \sum_{g=1}^{K_0} \|f^g\| \right)^2.
 \end{align}
 With $F_0=F_L=1$ and $F_l=F$ for $1\leq l\leq L-1$, then:
  \begin{align}
 \|y-y'\|^2 \leq LF^{L-1} C_{per}\epsilon  \|f\| .
 \end{align}
 \section{Proof of Proposition \ref{prop:finite_num}}
 Here we study the eigendecomposition in the Dirichlet condition. We have the following result for the spectrum of operator $\ccalL$ from results in \cite{berard2006spectral}.
\begin{theorem}\label{thm:eigenvalue}
Let $\ccalM$ be a compact manifold, consider the Dirichlet eigenvalue problems. Then:
\begin{enumerate}
    \item The set of eigenvalue consists of an infinite sequence $0<\lambda_1\leq \lambda_2\leq \lambda_3\leq \cdots \rightarrow \infty$;
    \item Each eigenvalue has finite multiplicity and the eigenspaces corresponding to distinct eigenvalues are $L^2(\ccalM)$-orthogonal;
\end{enumerate}
\end{theorem}

The spectrum cannot be calculated explicitly in general. However, it is still possible to get an estimation of the spectrum. The following Weyl's law gives a characterization of how the spectrum behaves asymptotically.
\begin{theorem}[Weyl's Law]\label{thm:Weyl_law}
If $(\ccalM,g)$ is a compact Riemannian manifold of dimension $d$, then
\begin{equation}\label{eqn:Weyllaw}
    \lambda_k(\ccalM,g)\sim \frac{4\pi^2}{C_d^{2/d}} \left( \frac{k}{\text{Vol}(\ccalM,g)} \right)^{2/d}
\end{equation}
as $k\rightarrow \infty$, and $C_d$ denotes the volume of the unit ball of $\reals^n$.
\end{theorem}

==> stability of NN on Rie-manifolds-eusipco/simulations.tex <==

We take a graph neural network model to approximate the manifold neural network. We verify our results on a {graph neural network} supported on a wireless adhoc network with $n=50$ nodes within a range of $[-50m,50m]^2$ where nodes are placed randomly. The channel states of all links can be represented by a matrix $\bbH(t)$ with each element $[\bbH(t)]_{ij}:=h_{ij}(t)$ denotes the channel condition between node $i$ and node $j$. Consider the large-scale pathloss gain and a random fast fading gain, this can be written as: $h_{ij}=\log( d_{ij}^{-2.2} h^f)$, where $d_{ij}$ stands for the distance between node $i$ and $j$, while $h^f\sim  \text{Rayleigh}(2)$ is the random fading. We here study the power allocation problem among $n$ nodes over an AWGN channel with interference, with $\bbp(\bbH)=[p_1(\bbH),p_2(\bbH),\hdots,p_n(\bbH)]$ denoting the power allocated to each node under channel condition $\bbH$. the channel rate of node $i$ is represented as $r_i$. The goal is to maximize the sum rate capacity under a total power budget $P_{max}$. This can be numerically formulated as:
\begin{align}
\label{eqn:prob_sim}
r^*&=\max_{\bbp(\bbH)} \sum_{i=1}^n r_i\\
   s.t.\quad \nonumber &r_i=\mathbb{E}\left[  \log\left(1+\frac{|h_{ii}|^2 p_i(\bbH)}{1+ \sum\limits_{j\neq i} |h_{ij}|^2 p_j(\bbH)}\right) \right],\\
   \nonumber & \mathbb{E}[\bm{1}^T\bbp]\leq P_{max},\quad p_i(\bbH)\in \{0,p_0\}.
\end{align}

With the nodes and the links seen as the graph nodes and edges respectively, the channel matrix $\bbH$ can be seen as a graph shift operator, more specifically, an adjacency matrix. By formulating $\bbH$ into a Laplacian matrix, the problem can be solved with a graph neural network composed with our defined $\alpha$-FDT filters with $\alpha$ set as 0.001. By setting $h_k=h_j$ for $|\lambda_k-\lambda_j|\leq\alpha$ in \eqref{eqn:operator}, we can get an approximation of $\alpha$-FDT filters. After trained for $4000$ iterations, the graph neural network can achieve the optimal power allocation.  In physical world, the nodes are deployed in some specific spatial positions. The positions may change and this would cause perturbations to the underlying Laplacian matrix. To model this, we add a log-normal matrix to the original channel matrix $\bbH$. With the same trained graph neural network employed, we measure the stability by the difference of final sum-rate. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{stability-eps-converted-to.pdf}
    \caption{Sum-rate difference on the test between the original wirelss network setting and the perturbed one.}
    \label{fig:sim_stability}
\end{figure}

We can observe from Figure \ref{fig:sim_stability} that the difference of the final sum-rates increases with the number of layers and the number of filters per layer in the neural network. This verifies the conclusion that we have derived in Theorem \ref{thm:stability_nn}.
